Linear Single-Source Shortest Path, Almost

We give a comparison--addition algorithm for single-source shortest paths in undirected graphs with nonnegative real edge lengths. For each input with $n$ vertices and $m$ edges, its expected running time is $O(m+n\log\log\log n)$. It terminates almost surely. Every terminating run returns exact distances and a shortest-path tree on the reachable vertices. The bound is independent of the ratio of edge lengths and is linear whenever $m=\Omega(n\log\log\log n)$. We also give randomized comparison--addition algorithms for exact global minimum cut in undirected graphs with arbitrary nonnegative real capacities. For every fixed positive integer $h$, one algorithm runs in worst-case time $O_h(m+n\log^{(h)}n)$, where $\log^{(h)}n$ is the lower-truncated $h$-fold logarithm; a uniform algorithm runs in worst-case time $O((m+n)2^{O(\log^* n)})$. Both bounds charge individually for every fair random bit, succeed with probability at least two thirds, and always return a nontrivial cut with its exact original capacity.

==> figures/graph-styles.tex <==
% Shared styles for graph vertices, edges, and diagram transitions.
\tikzset{
  paper graph vertex/.style={circle,draw=black!55,fill=white,
    line width=0.3pt,minimum size=4.1mm,inner sep=0pt,
    font=\fontsize{8.5}{10}\selectfont},
  paper graph edge/.style={line width=0.7pt,line cap=round,line join=round},
  paper graph arc/.style={paper graph edge,
    -{Latex[length=1.75mm,width=1.15mm]}},
  paper forest edge/.style={paper graph edge,line width=1.05pt},
  paper forest arc/.style={paper graph arc,paper forest edge},
  paper highlighted edge/.style={paper forest edge,line width=1.4pt},
  paper highlighted arc/.style={paper graph arc,paper highlighted edge,
    -{Latex[length=2mm,width=1.35mm]}},
  paper pending edge/.style={paper graph edge,draw=black!50,
    dash pattern=on 2.5pt off 1.7pt},
  paper step/.style={paper graph edge,
    -{Latex[length=2mm,width=1.35mm]}}
}


==> preamble.tex <==
% Formatting from arXiv:2610.13937v2 (CC0 1.0).
\usepackage{amsmath,amssymb,amsfonts,amsthm,mathtools}
\usepackage{thmtools}
\makeatletter
% Recent LaTeX kernels create shared theorem counters themselves.
\@ifundefined{newcounteralias}{}{%
  \renewcommand\thmt@autorefsetup{%
    \@xa\def\csname\thmt@envname autorefname\@xa\endcsname
      \@xa{\thmt@thmname}%
  }%
}
\IfFormatAtLeastTF{2024-11-01}{
  \renewcommand*\@addtoreset[2]{%
    \bgroup
      \edef\aliasctr@@truelist{\aliasctr@follow{#2}}%
      \let\@elt\relax
      \expandafter\@cons\aliasctr@@truelist{{#1}}%
    \egroup
    \expandafter\xdef\csname theH#1\endcsname{%
      \expandafter\noexpand\csname theH#2\endcsname.%
      \noexpand\the\noexpand\value{#1}}%
  }
}{}
\makeatother
\usepackage{thm-restate}

\usepackage[utf8]{inputenc}
\usepackage[T1]{fontenc}
\usepackage[tt=false, type1=true]{libertine}
\usepackage[varqu]{zi4}
\usepackage[libertine]{newtxmath}
\usepackage[margin=1in]{geometry}
\usepackage{microtype,parskip}
\usepackage{placeins}
\usepackage{float}

\usepackage{graphicx,xcolor}
\usepackage{booktabs,array,multirow,tabularx}

\usepackage[ruled,vlined]{algorithm2e}
\SetAlgoNoLine
\DontPrintSemicolon
\LinesNumbered
\SetKwComment{Comment}{\textcolor{blue}{// }}{}
\newcommand{\cmt}[1]{\Comment*[r]{\textcolor{blue}{#1}}}
\newcommand{\cmtl}[1]{\Comment*[l]{\textcolor{blue}{#1}}}

\usepackage{subcaption}
\captionsetup{subrefformat=parens}

\definecolor{ForestGreen}{rgb}{0.1333,0.5451,0.1333}
\definecolor{DarkRed}{rgb}{0.65,0,0}
\definecolor{LinkBlue}{rgb}{0.0,0.22,0.52}
\usepackage[bookmarks=true]{hyperref}
\hypersetup{
    colorlinks=true,
    linkcolor=DarkRed,
    filecolor=magenta,
    urlcolor=LinkBlue,
    citecolor=ForestGreen,
    linktocpage=true,
    bookmarksopen=true,
    bookmarksnumbered=true
}
\usepackage[nameinlink]{cleveref}
\usepackage{csquotes}
\usepackage[style=alphabetic,natbib=true,maxalphanames=3,minalphanames=3,maxbibnames=99,maxcitenames=3]{biblatex}
\addbibresource{references.bib}

\usepackage{tikz}
\usetikzlibrary{arrows.meta,positioning,calc,decorations.pathreplacing,matrix,patterns,decorations.pathmorphing,decorations.markings,fit}
\input{figures/graph-styles}

\usepackage{xspace,nicefrac}
\setcounter{tocdepth}{2}

\theoremstyle{plain}
\newtheorem{theorem}{Theorem}
\newtheorem{corollary}{Corollary}[section]
\newtheorem{lemma}[corollary]{Lemma}
\newtheorem{observation}[corollary]{Observation}
\newtheorem{proposition}[corollary]{Proposition}
\newtheorem{conjecture}[corollary]{Conjecture}
\newtheorem{claim}{Claim}[lemma]
\renewcommand{\theclaim}{\thelemma.\arabic{claim}}

\theoremstyle{definition}
\newtheorem{definition}[corollary]{Definition}
\newtheorem{example}[corollary]{Example}

\theoremstyle{remark}
\newtheorem{remark}[corollary]{Remark}

\usepackage{needspace,xurl}
\urlstyle{same}
\SetKwInput{KwIn}{Input}
\SetKwInput{KwOut}{Output}
\SetKw{Return}{return}
\SetKwProg{Fn}{Function}{}{}
\DeclareRobustCommand{\tref}[2]{\hyperref[#2]{#1~\ref*{#2}}}
\DeclareRobustCommand{\algcall}[2]{\hyperref[#1]{\textsc{#2}}~(\tref{Algorithm}{#1})}
\crefname{algocf}{algorithm}{algorithms}
\Crefname{algocf}{Algorithm}{Algorithms}
\crefname{observation}{observation}{observations}
\Crefname{observation}{Observation}{Observations}
\setlength{\emergencystretch}{2em}
\newcommand{\E}{\mathbb E}
\newcommand{\Prb}{\mathbb P}
\newcommand{\lamtwo}{\lambda_2}
\newcommand{\LCA}{\operatorname{LCA}}

